MMCR4NLP: Multilingual Multiway Corpora Repository for Natural Language Processing

Multilinguality is gradually becoming ubiquitous in the sense that more and more researchers have successfully shown that using additional languages help improve the results in many Natural Language Processing tasks. Multilingual Multiway Corpora (MMC) contain the same sentence in multiple languages. Such corpora have been primarily used for Multi-Source and Pivot Language Machine Translation but are also useful for developing multilingual sequence taggers by transfer learning. While these corpora are available, they are not organized for multilingual experiments and researchers need to write boilerplate code every time they want to use said corpora. Moreover, because there is no official MMC collection it becomes difficult to compare against existing approaches. As such we present our work on creating a unified and systematically organized repository of MMC spanning a large number of languages. We also provide training, development and test splits for corpora where official splits are unavailable. We hope that this will help speed up the pace of multilingual NLP research and ensure that NLP researchers obtain results that are more trustable since they can be compared easily. We indicate corpora sources, extraction procedures if any and relevant statistics. We also make our collection public for research purposes.

==> additional.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[]
\begin{center}
\setlength{\tabcolsep}{.2em}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
Language                                                            & Ar    & Fr    & Es    & Zh & Ru    & En    \\ \hline
\begin{tabular}[c]{@{}c@{}}Line\\ Count\end{tabular}                & \multicolumn{6}{c|}{11.36}                 \\ \hline
\begin{tabular}[c]{@{}c@{}}Word\\ Count\end{tabular}                & 262.7 & 339.4 & 350.1 & -  & 273.2 & 294.4 \\ \hline
\begin{tabular}[c]{@{}c@{}}Unique \\ Word\\ Count\end{tabular}      & 2.47  & 1.48  & 1.59  & -  & 2.24  & 1.64  \\ \hline
\begin{tabular}[c]{@{}c@{}}Average\\ Sentence\\ Length\end{tabular} & 23    & 29    & 30    & -  & 24    & 25    \\ \hline
\end{tabular}
\caption{Corpora statistics for the United Nations 6 lingual corpus.}
\label{uncorpus}
\end{center}
\end{table}

\begin{table}[]
\centering
\resizebox{\textwidth}{!}{%
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
Language &  & Da & De & Es & Pt & It & Nl & Fr & Fi & Sv & En & Hu & Lt & Lv & Bg & El & Et & Ro & Sk & Sl & Cs & Pl \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Line\\ Count\end{tabular}} & 21-way & \multicolumn{21}{c|}{0.189} \\ \cline{2-23} 
 & 10-way & \multicolumn{10}{c|}{1.07} & \multicolumn{11}{c|}{-} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Word\\ Count\end{tabular}} & 21-way & 4.66 & 4.79 & 5.40 & 5.15 & 4.91 & 5.23 & 5.36 & 3.44 & 4.57 & 5.07 & 4.16 & 3.76 & 3.92 & 4.76 & 5.12 & 3.62 & 5.02 & 4.22 & 4.24 & 4.21 & 4.24 \\ \cline{2-23} 
 & 10-way & 25.84 & 26.29 & 29.67 & 28.65 & 27.26 & 28.76 & 29.52 & 19.15 & 25.61 & 28.19 & \multicolumn{11}{c|}{-} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Unique \\ Word Count\end{tabular}} & 21-way & 0.145 & 0.162 & 0.114 & 0.120 & 0.122 & 0.127 & 0.109 & 0.274 & 0.147 & 0.083 & 0.269 & 0.206 & 0.169 & 0.138 & 0.143 & 0.247 & 0.129 & 0.175 & 0.164 & 0.179 & 0.188 \\ \cline{2-23} 
 & 10-way & 0.462 & 0.473 & 0.311 & 0.326 & 0.334 & 0.375 & 0.307 & 0.856 & 0.463 & 0.228 & \multicolumn{11}{c|}{-} \\ \hline
\multirow{2}{*}{\begin{tabular}[c]{@{}c@{}}Avg Sent\\ Length\end{tabular}} & 21-way & 24 & 25 & 28 & 27 & 25 & 27 & 28 & 18 & 24 & 26 & 22 & 19 & 20 & 25 & 27 & 19 & 26 & 22 & 22 & 22 & 22 \\ \cline{2-23} 
 & 10-way & 24 & 24 & 27 & 26 & 25 & 26 & 27 & 17 & 23 & 26 & \multicolumn{11}{c|}{-} \\ \hline
\end{tabular}%
}
\caption{Corpora statistics for the Europarl 21 lingual corpus.}
\label{my-label}
\end{table}
